Core Higher-Order Session Processes: Tractable Equivalences and Relative Expressiveness

This work proposes tractable bisimulations for the higher-order pi-calculus with session primitives (HOpi) and offers a complete study of the expressivity of its most significant subcalculi. First we develop three typed bisimulations, which are shown to coincide with contextual equivalence. These characterisations demonstrate that observing as inputs only a specific finite set of higher-order values (which inhabit session types) suffices to reason about HOp} processes. Next, we identify HO, a minimal, second-order subcalculus of HOpi in which higher-order applications/abstractions, name-passing, and recursion are absent. We show that HO can encode HOpi extended with higher-order applications and abstractions and that a first-order session pi-calculus can encode HOpi. Both encodings are fully abstract. We also prove that the session pi-calculus with passing of shared names cannot be encoded into HOpi without shared names. We show that HOpi, HO, and pi are equally expressive; the expressivity of HO enables effective reasoning about typed equivalences for higher-order processes.

==> contribution.tex <==
\section*{\dk{TODO list}}
\begin{enumerate}
	\item	Operational Correspondence: \HOp to \sessp.
	\item	Type Preservation: \HOpp to \HOp: Do some proof cases.
	\item	Operational Correspondence: \pHOp to \HOp: Do some proof cases
%	\item	Full Abstraction: \pHOp to \HOp.
	\item	Revise related work wrt to LICS version.
	\item	Review Appendix
\end{enumerate}


==> figures/fig-aux_encoding.tex <==
\begin{figure}[t]
\[
	\begin{array}{rcl}
		\auxmap{\news{n} P}{\sigma} &\bnfis& \news{n} \auxmap{P}{{\sigma \cat n}}
		\vspace{1mm} \\

		\auxmap{\bout{n}{\abs{x}{Q}} P}{\sigma} &\bnfis&
		\left\{
		\begin{array}{rl}
			\bout{x_n}{\abs{x}{\auxmap{Q}{\sigma}}} \auxmap{P}{\sigma} & n \notin \sigma\\
			\bout{n}{\abs{x}{\auxmap{Q}{\sigma}}} \auxmap{P}{\sigma} & n \in \sigma
		\end{array}
		\right.
		\vspace{1mm}	\\ 

		\auxmap{\binp{n}{X} P}{\sigma} &\bnfis&
		\left\{
		\begin{array}{rl}
			\binp{x_n}{X} \auxmap{P}{\sigma} & n \notin \sigma\\
			\binp{n}{X} \auxmap{P}{\sigma} & n \in \sigma
		\end{array}
		\right.

		\vspace{1mm}	\\ 
		\auxmap{\bsel{n}{l} P}{\sigma} &\bnfis&
		\left\{
		\begin{array}{rl}
			\bsel{x_n}{l} \auxmap{P}{\sigma} & n \notin \sigma\\
			\bsel{n}{l} \auxmap{P}{\sigma} & n \in \sigma
		\end{array}
		\right.
		\vspace{1mm} \\
		\auxmap{\bbra{n}{l_i:P_i}_{i \in I}}{\sigma} &\bnfis&

		\left\{
		\begin{array}{rl}
			\bbra{x_n}{l_i:\auxmap{P_i}{\sigma}}_{i \in I}  & n \notin \sigma\\
			\bbra{n}{l_i:\auxmap{P_i}{\sigma}}_{i \in I}  & n \in \sigma
		\end{array}
		\right.
		\vspace{1mm} \\
		\auxmap{\appl{x}{n}}{\sigma} &\bnfis&
		\left\{
		\begin{array}{rl}
			\appl{x}{x_n} & n \notin \sigma\\
			\appl{x}{n} & n \in \sigma\\
		\end{array}
		\right.
		\vspace{1mm} \\

		\auxmap{\inact}{\sigma} &\bnfis& \inact
		\vspace{1mm} \\

		\auxmap{P \Par Q}{\sigma} &\bnfis& \auxmap{P}{\sigma} \Par \auxmap{Q}{\sigma}
	\end{array}
\]
\caption{\label{fig:auxmap} The auxiliary map (cf. Def.~\ref{def:auxmap}) 
used in the encoding of the recursive primitives of \HOp into \HO (Def.~\ref{def:enc:HOp_to_HO}).}
\end{figure}


